Scalable multiscale-spectral GFEM with an application to composite aero-structures

In this paper, the first large-scale application of multiscale-spectral generalized finite element methods (MS-GFEM) to composite aero-structures is presented. The crucial novelty lies in the introduction of A-harmonicity in the local approximation spaces, which in contrast to [Babuska, Lipton, Multiscale Model. Simul. 9, 2011] is enforced more efficiently via a constraint in the local eigenproblems. This significant modification leads to excellent approximation properties, which turn out to be essential to capture accurately material strains and stresses with a low dimensional approximation space, hence maximising model order reduction. The implementation of the framework in the DUNE software package, as well as a detailed description of all components of the method are presented and exemplified on a composite laminated beam under compressive loading. The excellent parallel scalability of the method, as well as its superior performance compared to the related, previously introduced GenEO method are demonstrated on two realistic application cases, including a C-shaped wing spar with complex geometry. Further, by allowing low-cost approximate solves for closely related models or geometries this efficient, novel technology provides the basis for future applications in optimisation or uncertainty quantification on challenging problems in composite aero-structures.

==> GenEO online-offline + MLMCMC/glossary.tex <==
\newacronym{UQ}{UQ}{Uncertainty Quantification}
\newacronym{MC}{MC}{Monte Carlo}
\newacronym{MCMC}{MCMC}{Markov chain Monte Carlo}
\newacronym{MLMCMC}{MLMCMC}{Multilevel Markov chain Monte Carlo}
\newacronym{MLMC}{MLMC}{Multilevel Monte Carlo}
\newacronym{HPC}{HPC}{High Performance Computing}
\newacronym{DUNE}{DUNE}{Distributed and Unified Numerics Environment}
\newacronym{GMsFEM}{GMsFEM}{Generalized Multiscale Finite Element Method}
\newacronym{GEVP}{GEVP}{generalized eigenvalue problem}
\newacronym{MS-GFEM}{MS-GFEM}{multiscale-spectral generalized finite element method}
\newacronym{ATI}{ATI}{Aerospace Technology Institute}
\newacronym{GenEO}{GenEO}{Generalized Eigenproblems in the Overlaps}
\newacronym{A-h-GenEO}{A-h-GenEO}{A-harmonic GenEO}
\newacronym{FE}{FE}{finite element}
\newacronym{DoF}{DoF}{degree of Freedom}
\newacronym{PDE}{PDE}{partial differential equation}
\newacronym{LMOR}{LMOR}{localized model order reduction}
\newacronym{UMFPACK}{UMFPACK}{Unsymmetric MultiFrontal PACKage}
\newacronym{CG}{CG}{Conjugate Gradient}
\newacronym{GMRES}{GMRES}{Generalized Minimal Residual}
\newacronym{AMG}{AMG}{Algebraic Multigrid}
\newacronym{DD}{DD}{Domain Decomposition}
\newacronym{MAP}{MAP}{Maximum a Posteriori Probability}
\newacronym{o}{o}{overlap size}
\newacronym{ovs}{ovs}{oversampling size}
\newacronym{REV}{REV}{representative elementary volume}
\newacronym{PoU}{PoU}{partition of unity}

